On Model Identification and Out-of-Sample Prediction of Principal Component Regression: Applications to Synthetic Controls

We analyze principal component regression (PCR) in a high-dimensional error-in-variables setting with fixed design. Under suitable conditions, we show that PCR consistently identifies the unique model with minimum $\ell_2$-norm. These results enable us to establish non-asymptotic out-of-sample prediction guarantees that improve upon the best known rates. In the course of our analysis, we introduce a natural linear algebraic condition between the in- and out-of-sample covariates, which allows us to avoid distributional assumptions for out-of-sample predictions. Our simulations illustrate the importance of this condition for generalization, even under covariate shifts. Accordingly, we construct a hypothesis test to check when this conditions holds in practice. As a byproduct, our results also lead to novel results for the synthetic controls literature, a leading approach for policy evaluation. To the best of our knowledge, our prediction guarantees for the fixed design setting have been elusive in both the high-dimensional error-in-variables and synthetic controls literatures.

==> content/abstract.tex <==
We analyze principal component regression (PCR) in a high-dimensional error-in-variables setting with fixed design.
%
Under suitable conditions, we show that PCR consistently identifies the unique model with minimum $\ell_2$-norm. 
% and is near minimax optimal. 
%
These results enable us to establish non-asymptotic out-of-sample prediction guarantees that improve upon the best known rates. 
%
In the course of our analysis, we introduce a natural linear algebraic condition between the in- and out-of-sample covariates, which allows us to avoid distributional assumptions for out-of-sample predictions. 
% 
Our simulations illustrate the importance of this condition for generalization, even under covariate shifts. 
%
Accordingly, we construct a hypothesis test to check when this conditions holds in practice. 
%
As a byproduct, our results also lead to novel results for the synthetic controls literature, a leading approach for policy evaluation. 
%
%In particular, our minimax results suggest the attractiveness of PCR based methods amongst the numerous variants. 
% 
To the best of our knowledge, our prediction guarantees for the fixed design setting have been elusive in both the high-dimensional error-in-variables and synthetic controls literatures. 
%







==> content/figures.tex <==
\clearpage 
\section{Figures}

% \begin{figure} [!h]
%      \centering
%      \includegraphics[width=0.40\linewidth]
%      {images/elbow.jpg}
%      \caption{
%      {\smaller
%      %
%      We plot the spectrum of $\bZ = \bX + \bW \in \Rb^{100 \times 100}$. 
%      %
%      $\bX = \bU \bV^T$, where entries of $\bU, \bV \in \Rb^{100 \times 10}$ are sampled independently from $\mathcal{N}(0,1)$;  
%      entries of $\bW$ are sampled independently from $\mathcal{N}(0, \sigma^2)$ with $\sigma^2 \in \{0, 0.2, \dots, 0.8\}$. 
%      %
%      We see a steep drop-off in magnitude from the top to remaining singular values across all noise levels---this marks the ``elbow'' point. 
%      %
%      Top singular values of $\bZ$ correspond closely with those of $\bX$ ($\sigma^2=0$). The remaining singular values are induced by $\bW$.
%      %
%      Thus, $\rank(\bZ) \approx \rank(\bX) = 10$.
%      %
%      }
%      }
%      \label{fig:elbow}
%  \end{figure}
 
%  \begin{figure} [!b] 
% 	\centering
% 	\begin{subfigure}[t]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{images/pe_final1.png}%{a}
% 		\caption{{\smaller $\ell_2$-norm error of $\bhbeta$ with respect to min. $\ell_2$-norm solution of \eqref{eq:response_vector}.}
% 		\label{fig:param_est.1}}
% 	\end{subfigure}
% 	\hspace{5mm}
% 	\begin{subfigure}[t]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\linewidth]{images/pe_final2.png}%{a}
% 		\caption{{\smaller$\ell_2$-norm error of $\bhbeta$ with respect to a random solution of \eqref{eq:response_vector}.}}
% 		\label{fig:param_est.2}
% 	\end{subfigure}
% 	\caption{{\smaller Plots of $\ell_2$-norm errors, i.e., $\| \bhbeta - \btbeta^* \|_2$ in (\ref{fig:param_est.1}) and $\|\bhbeta - \bbeta^* \|_2$ in (\ref{fig:param_est.2}), versus the rescaled sample size $n / (r^2 \log p)$ after running PCR with rank $r = p^{\frac 13}$. As predicted by Theorem \ref{thm:param_est}, the curves for different values of $p$ under (\ref{fig:param_est.1}) roughly align and decay to zero as $n$ increases.}}
% 	\label{fig:param_est_full}
% \end{figure}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.45\linewidth]{images/pcr_distribution_shift.png}
% 	\caption{
% 	    %
% 	    MSE plot of multiple PCR estimates as we shift the distribution of the out-of-sample covariates, while ensuring Assumption \ref{assumption:subspace_incl} holds. The MSE remains closely matched across all noise levels and distribution shifts.
% 	}
% 	\label{fig:pcr_distribution_shift}
% \end{figure}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.45\linewidth]{images/subspace_v_iid5.png}
% 	\caption{
% 	   {
% 	    %
% 	    Plots of PCR's MSE under two cases: Assumption \ref{assumption:subspace_incl} holds but distributional invariance is violated (blue), and Assumption \ref{assumption:subspace_incl} is violated but distributional invariance holds (orange).
% 	    Across varying levels of noise, the former condition achieves a much lower MSE.
% 	    }
% 	}
% 	\label{fig:subspace_v_iid}
% \end{figure}


==> content/notation.tex <==
% NOTATION
\section{Notation} 
%
For any matrix $\bA \in \Rb^{a \times b}$, we denote its operator (spectral), Frobenius, and max element-wise norms as $\|\bA\|_{2}$, $\|\bA\|_F$, and $\|\bA\|_{\max}$, respectively. 
%
By $\text{rowspan}(\bA)$, we denote the
subspace of $\Rb^b$ spanned by the rows of $\bA$.
%
For any vector $\bv \in \Rb^a$, let $\|\bv\|_p$ denote its 
$\ell_p$-norm.
%
We define the sub-gaussian (Orlicz) norm of a random $\bv$ as $\|\bv\|_{\psi_2}$. 
%
Let $\circ$ denote component-wise multiplication and let $\otimes$ denote the outer product.
For any two numbers $a, b \in\Rb$, we use $a \wedge b$ to denote $\min(a, b)$ and $a \vee b$ to denote $\max(a, b)$. 
Further, let $[a] = \{1, \dots, a\}$ for any integer $a$.
%
%
Let $f$ and $g$ be two functions defined on the same space. We say that $f(n)$ = $O(g(n))$ if and only if
there exists a positive real number $M$ and a real number $n_0$ such that for all $n \ge n_0, |f (n)| \le M|g(n)|$.
%
Analogously we say
$f (n) = \Theta(g(n))$ if and only if there exists positive real numbers $m, M$ such that for all $n \ge n_0, \ m|g(n)| \le |f(n)| \le M|g(n)|$;
%
$f (n) = o(g(n))$ if for any $m > 0$, there exists $n_0$ such that for all 
$n \ge n_0, |f(n)| \le m|g(n)|$;
%
$f (n) = \omega(g(n))$ if for any $m > 0$, there exists $n_0$ such that for all 
$n \ge n_0, |f(n)| \ge m|g(n)|$.
%
$\tO(\cdot)$ is defined analogously to $O(\cdot)$, but ignores $\log$ dependencies.

